Optimizing Functionals on the Space of Probabilities with Input Convex Neural Networks

Gradient flows are a powerful tool for optimizing functionals in general metric spaces, including the space of probabilities endowed with the Wasserstein metric. A typical approach to solving this optimization problem relies on its connection to the dynamic formulation of optimal transport and the celebrated Jordan-Kinderlehrer-Otto (JKO) scheme. However, this formulation involves optimization over convex functions, which is challenging, especially in high dimensions. In this work, we propose an approach that relies on the recently introduced input-convex neural networks (ICNN) to parametrize the space of convex functions in order to approximate the JKO scheme, as well as in designing functionals over measures that enjoy convergence guarantees. We derive a computationally efficient implementation of this JKO-ICNN framework and experimentally demonstrate its feasibility and validity in approximating solutions of low-dimensional partial differential equations with known solutions. We also demonstrate its viability in high-dimensional applications through an experiment in controlled generation for molecular discovery.

==> backup/experiments.bak.tex <==
\section{Evolving PDEs with known solutions}\label{sec:experiments_pde}

\begin{figure*}
     \centering
     \begin{subfigure}[b]{\textwidth}
         \centering
        \includegraphics[height=3.1cm, trim={0.2cm 0.2cm 0.2cm 0.2cm}, clip]{images/pme_exact_density.png}%    
        \includegraphics[height=3.1cm, trim={0.2cm 0.2cm 0.2cm 0.2cm}, clip]{images/pme_t0.001_it1000_strNone_density.png}%
        \includegraphics[height=3.1cm, trim={0.2cm 0.2cm 0.2cm 0.2cm}, clip]{images/pme_t0.001_it1000_strNone_F_convergence.png}%
        \includegraphics[height=3.1cm, trim={0.2cm 0.2cm 0.2cm 0.2cm}, clip]{images/pme_t0.001_it1000_strNone_convergence.png}%    
        \caption{Porous medium equation with pure diffusion \sref{sec:results_pme}.}
         \label{fig:1d_pde_pme}
     \end{subfigure}
     \begin{subfigure}[b]{0.495\textwidth}
         \centering
        \includegraphics[height=3.1cm, trim={0.2cm 0.2cm 0.2cm 0.2cm}, clip]{images/fplanck_t0.01_it1000_strNone_rho_convergence.png}%
        \includegraphics[height=3.1cm, trim={0.2cm 0.2cm 0.2cm 0.2cm}, clip]{images/fplanck_t0.01_it1000_strNone_F_convergence.png}
        \caption{Fokker-Planck with nonlinear diffusion \sref{sec:results_fokkerplanck}.}
         \label{fig:1d_pde_fp}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.495\textwidth}
         \centering
        \includegraphics[height=3.1cm, trim={0.2cm 0.2cm 0.2cm 0.2cm}, clip]{images/aggregation_averaged_t_1.0.png}%
        \includegraphics[height=3.1cm, trim={0.2cm 0.2cm 0.2cm 0.2cm}, clip]{images/aggregation_F_convergence_t_1.0.png}
        \caption{Aggregation equation \sref{sec:results_aggregation}.}
         \label{fig:1d_pde_agg}
     \end{subfigure}
     \caption{\textbf{Flows on PDEs with known solution.} We use KDE on the flowed particles for the density plots, and the iterated push-forward density method (Corollary \ref{cor:IteratedDensity}) to evaluate $\cF$ in (a) and (b).}
     \label{fig:1d_pde}
\end{figure*}

We first evaluate our method on gradient flows whose corresponding PDEs have known solutions. We focus on three examples from \citet{carrillo2021primal} that combine the three types of functionals considered here (\sref{sec:grad_flows}): porous medium, non-linear Fokker-Planck, and aggregation equations.
We also compare in Figure \ref{fig:pde_flow_comparison} in Appendix \ref{app:WFhighdim} the dynamics of JKO-ICNN and Langevin dynamics at  recovering the Wasserstein gradient flow corresponding to the Fokker-Planck equation in high dimension $(\R^{20})$. Throughout this section, we use $\tau\!=\!\eta\!=\!10^{-3}$ in the notation of Algorithm~\ref{alg:JKO-ICNN}. 

\subsection{Porous medium equation}\label{sec:results_pme}
The porous medium equation is a classic non-linear diffusion PDE. We consider in particular a diffusion-only system: $\partial_t\rho = \Delta \rho^m, m>1$, corresponding to a gradient flow of the internal energy functional $\cF(\rho)=\frac{1}{m-1}\int \rho^m(x) \dif x$, which we implement using our JKO-ICNN with objective~\eqref{eq:nonlin_diff_surrogate}. A known family of exact solutions of this PDE is given by the Barenblatt-Pattle profiles \citep{zeldovich1950towards, barenblatt1952some, pattle1959diffusion}:
\vspace{-0.2cm}
\[ \rho(x,t) = t^{-\alpha} \bigl( C - k \|x\|^2 t^{-2\beta} \bigr)^{\frac{1}{m-1}}_{+}\!, \quad x\in \R^d, \medspace t >0, \vspace{-0.2cm}\]
where $C\!>\!0$ is a constant and $\alpha = d/(d(m-1) +2)$, $\beta=\alpha/d$, and $k = \alpha(m-1)/(2md)$. 

This exact solution provides a trajectory of densities to compare our JKO-ICNN approach against. Specifically, starting from particles sampled from $\rho(x,0)$, we can compare the trajectory $\hat{\rho}_t(x)$ estimated with our method to the exact density $\rho(x,t)$. Although this system has no steady-state solution, its asymptotic behavior can be expressed analytically too. For the case $d\!=\!1,m\!=\!2, C=(\sfrac{3}{16})^{1/3}$, Figure~\ref{fig:1d_pde_pme} shows that our method reproduces the dynamics of the exact solution (here the flow density is estimated from particles via KDE and aggregated over 10 repetitions with random initialization), and that the objective value $\cF(\hat{\rho})$ has the correct asymptotic behavior. \looseness=-1

\subsection{Nonlinear Fokker-Planck equation}\label{sec:results_fokkerplanck}
Next, we consider a Fokker-Planck equation with a non-linear diffusion term as before:
\begin{equation}
    \partial_t \rho = \nabla \cdot (\rho \nabla V) + \Delta \rho^m,  \quad V: \R^d \rightarrow \R, \quad m>1.
\end{equation}
This PDE corresponds to a gradient flow of the objective ${F}(\rho) = \frac{1}{m-1}\int \rho^m(x) \dif x + \int V(x)\dif \rho(x)$. For some $V$'s its solutions approach a unique steady state \citep{carrillo2000asymptotic}:
\begin{equation}
    \rho_{\infty}(x) = \bigl(C - \tfrac{m-1}{m}V(x) \bigr)_{+}^{\frac{1}{m-1}},
\end{equation}
where the constant $C$ depends on the initial mass of the data. For $d\!=\!1$, $m\!=\!2$, and $V(x)\!=\!x^2$, we solve this PDE using JKO-ICNN with objectives \eqref{eq:v_w_expectations} and \eqref{eq:nonlin_diff_surrogate}, using initial data drawn from a Normal distribution with parameters $(\mu,\sigma^2)=(0,0.2)$. Unlike the previous example, in this case we do not have a full solution $\rho(x,t)$ to compare against, but we can instead evaluate convergence of the flow to $\rho_{\infty}(x)$. Figure~\ref{fig:1d_pde_fp} shows that the density $\hat{\rho}_t(x)$ derived from the JKO-ICNN flow converges to the steady state $\rho_{\infty}(x)$, and so does the value of the objective, i.e., ${F}(\hat{\rho_t}) \rightarrow {F}(\rho_{\infty})$. 

\subsection{Aggregation equation}\label{sec:results_aggregation}
Next, we consider an aggregation equation: $    \partial_t \rho  = \nabla \cdot (\rho \nabla W\ast \rho), W:\R^d \rightarrow \R$,
% \begin{equation}
%     \partial_t \rho  = \nabla \cdot (\rho \nabla W\ast \rho), \quad  W:\R^d \rightarrow \R, 
% \end{equation}
which corresponds to a gradient flow on an interaction functional $\mathcal{W}(\rho)=\frac{1}{2}\iint W(x-x')\dif \rho(x)\dif \rho(x')$. We consider the same setting as \citet{carrillo2021primal}: $d\!=\!1$, $\rho_0 \sim \cN(0,1)$, and the kernel $W(x) = \tfrac{1}{2} |x|^2 - \log (|x|)$, which enforces repulsion at short length scales and attraction at longer scales. This choice of $W$ has the advantage of yielding a unique steady-state equilibrium \citep{carrillo2012mass}, given by $\rho_{\infty}(x) = \frac{1}{\pi} \sqrt{(2-x^2)_{+}}$.
% \[ \rho_{\infty}(x) = \frac{1}{\pi} \sqrt{(2-x^2)_{+}}\]
Our JKO-ICNN encodes $\cW$ using the objective \eqref{eq:v_w_expectations}. As in the previous section, we investigate the convergence of this flow to this steady state distribution. Figure~\ref{fig:1d_pde_agg} shows that in this case too we observe convergence of densities $\hat{\rho}_t(x) \rightarrow \rho_{\infty}(x)$ and objective values $F(\hat{\rho_t}) \rightarrow F(\rho_{\infty})$. 


\section{Molecular discovery}\label{sec:experiments_molecules}

To demonstrate the flexibility and efficacy of our approach, we apply it in an important high dimensional setting: controlled generation in molecular discovery.
For the reader less familiar with molecular generation, this application is analogous to conditional image generation and editing.
In our experiments, our goal is to increase the \textit{drug-likeness} of a given distribution of molecules while staying close to the original distribution, an important task in drug discovery and drug re-purposing.
Formally, given an initial distributions of molecules $\rho_0$ and a convex potential energy function $V(\cdot)$ that models the property of interest, we wish to solve:
\begin{equation}
\min_{\rho \in \mathcal{P}(\mathcal{X})} {F}(\rho):=\lambda_1 \mathbb{E}_{\rho} V(x)+ \lambda_2 \textup{D}(\rho,\rho_0), 
\label{eq:MolDis}
\end{equation}
where $\textup{D}$ is a divergence.
In particular, we use either the 2-Wasserstein distance with entropic regularization \citep{cuturi2013sinkhorn} or the Maximum Mean Discrepancy \citep{MMD} with a Gaussian kernel ($\mathrm{MMD}$).
Finally, we use our JKO-ICNN scheme (Algorithm \ref{alg:JKO-ICNN}) to optimize this functional on the space of probability measures, given an initial distribution $\rho_0(x)= \frac{1}{N}\sum_{i=1}^N \delta_{x_i}(x)$ where $x_i$ is a molecular embedding. 

In what follows, we show how we model each component of this functional via : i) training a molecular embedding using a Variational Auto-encoder (VAE), ii) training a surrogate potential $V$ to model the drug-likeness, iii) using automatic differentiation via the divergence $\textup{D}$.    

\begin{remark}
Note that in Equation \ref{eq:MolDis}, since $V$ is convex, the objective functional is geodesically convex for $D$ being the $2$- Wasserstein distance and hence a solution exists for the JKO scheme \cite{santambrogio2017euclidean}. By using an entropic regularization, with $\textup{D}$ being the Sinkhorn divergence, we are therefore approximating this solution. For $\textup{D}$ being the MMD, the problem is not geodesically convex.     
\end{remark}
\paragraph{Embedding of molecules using VAEs} We start by training a VAE on string representation of molecules \cite{10.3389/fphar.2020.565644, chenthamarakshan2020cogmol} known as SMILES \cite{weininger1988smiles} to reconstruct these strings with a regularization term that ensures smoothness of the encoder's latent space \cite{kingma2013auto, higgins2016beta}.
We train the VAE on a molecular dataset known as MOSES \cite{10.3389/fphar.2020.565644}, which is a subset of the ZINC database \cite{sterling2015zinc}, released under the MIT license.
This dataset contains about 1.6M training and 176k test molecules.
Given a molecule, we embed it using the encoder of the VAE and represent it with a vector $x_i \in \mathbb{R}^{128}$.
See Appendix \ref{app:qm9}, where we also present results for the experiment run on the popular QM9 dataset \cite{ramakrishnan2014quantum, ruddigkeit2012enumeration}.

\paragraph{Training a convex surrogate for the desired property (high QED)}

The quantitative estimate of drug-likeness (QED) \citep{bickerton2012quantifying} can be computed with the RDKit library \cite{landrum2013rdkitsoftware, landrum2013rdkit} but is not differentiable nor convex.
Hence, we propose to learn a convex surrogate using Residual ICNNs \cite{amos2017input, huang2021convex}.
This ensures that it can be used as convex potential functional $\mathcal{V}$, as described in Section \ref{sec:grad_flows}.
To do so we process the MOSES dataset via RDKit and obtain a labeled set with all QED values.
We set a QED threshold of 0.85 and give a lower value label for all QED values above that threshold and a higher value label for all QED values below it so that minimizing the potential functional with this convex surrogate will lead to higher QED values.
Given VAE embeddings of the molecules, we train a ICNN classifier on this dataset.
%This results in a surrogate potential $V$ that has low energy on molecules with high QED $(>0.85)$.
See Appendix \ref{app:mol-pde} for experimental details. %about the hyperparameters and performance of the Residual ICNN that was trained as the QED classifier.

\paragraph{Automatic differentiation via $\textup{D}$} When $\textup{D}$ is the entropy-regularized Wasserstein distance, we use the Sinkhorn algorithm \cite{cuturi2013sinkhorn} to compute it (and henceforth denote it as $\mathrm{Sinkhorn}$). We backpropagate through this objective as proposed by \citet{genevay2018learning}, using the \texttt{geomloss} toolbox for efficiency \citep{feydy2019interpolating}.
We also use \texttt{geomloss} for evaluation and backpropagation when $\textup{D}$ is chosen to be $\mathrm{MMD}$.
\begin{figure}[ht!]
    \centering
    \vspace{-0.4cm}    
    \includegraphics[width=0.9\columnwidth]{images/mol_pde_final.pdf}
    \caption{\textbf{JKO-ICNN for molecular discovery.}
    We apply our method to generate molecules whose drug-likeness and closeness to $\rho_0$ are maximized in latent VAE space.} %domain by combining the convex QED classifier potential with a distributional distance.}
    \label{fig:mol_pde_setup}
\vskip -0.12in
\end{figure}
\paragraph{Optimization with JKO} With the molecule embeddings coming from the VAE serving as the point cloud to be transported and the potential functional defined by the convex QED classifier, we run Algorithm \ref{alg:JKO-ICNN} to move an initial point cloud of molecule embeddings $\rho_0$ with low drug-likeness (QED < 0.7) to a region of the latent space that decodes to molecules with distribution 
$\rho^{T}_{\tau}$ with higher drug-likeness.
The divergence $\textup{D}$ between the initial point cloud and subsequent point clouds of embeddings allows us to control for other generative priorities, such as staying \textit{close} to the original set of molecules.
Following the notation of Algorithm \ref{alg:JKO-ICNN}, we used the following hyperparameters for the JKO-ICNN in this setting.
$N$, number of original embeddings, was 1,000.
The JKO rate $\tau$ was set to $1\rm{e}^{-4}$ and the outer loop steps $T$ was set to 100.
For the inner loop, the number of iterations $n_u$ was set to 500, and the inner loop learning rate $\eta$ was set to $1\rm{e}^{-3}$.
For the JKO $\rm{ICNN}$, we used a fully-connected ICNN with two hidden layers, each of dimension 100.
Finally, we ran the JKO-ICNN flow without warm starts between steps.
The full pipeline for this experiment setting is displayed in Figure \ref{fig:mol_pde_setup}.
All computation for this pipeline,
was done in a compute environment with 1 CPU and 1 V100 GPU submitted as resource-restricted jobs to a cluster.

% %\paragraph{From ICNN JKO Solution  back to Molecules.} Decoder
\iffalse
\youssef{move table 2  to appendix}
\begin{table*}[ht!]
\vskip -0.1in
    \centering
    \caption{\textbf{Molecular discovery results.}
    Measures of validity, uniqueness, and median QED are reported in each row for the corresponding point cloud of embeddings.
   % For each point cloud, we decode the embeddings to get SMILES strings and use RDKit to determine whether the corresponding string is valid and get the associated QED value.
    The first row shows these metrics for the initial dataset, and the subsequent rows correspond to the datasets obtained with JKO-ICNN for different  $\textup{D}$ ($\mathrm{Sinkhorn}$ or $\mathrm{MMD}$) and weight parameter $\lambda_2$. Each measurement value cell contains mean values $\pm$ one standard deviation for $5$ repeated runs  with different random initialization seeds.
    %We find that the setup that uses
    Using $\mathrm{Sinkhorn}$ with weight 10,000 yields improved  QED (higher is better) without sacrificing validity and uniqueness of the decoded SMILES strings.}
    \begin{tabular}{l l l | c c c}
    \toprule
    Measure & $\textup{D}$ & $\lambda_2$ & Validity & Uniqueness & QED Median\\
    \midrule
    $\rho_0$ & N/A & N/A & 100.000 $\pm$ 0.000 & 99.980 $\pm$ 0.045 & 0.630 $\pm$ 0.001\\
    \midrule\midrule
    $\rho^{\tau}_{T}$ & $\mathrm{Sinkhorn}$ & 1,000 & 92.460 $\pm$ 2.096 & 69.919 $\pm$ 4.906 & 0.746 $\pm$ 0.016\\
    $\rho^{\tau}_{T}$ & $\mathrm{Sinkhorn}$ & 10,000 & 93.020 $\pm$ 1.001 & 99.245 $\pm$ 0.439 & 0.769 $\pm$ 0.002\\
    $\rho^{\tau}_{T}$ & $\mathrm{MMD}$ & 1,000 & 94.560 $\pm$ 1.372 & 51.668 $\pm$ 2.205 & 0.780 $\pm$ 0.009\\
    $\rho^{\tau}_{T}$ & $\mathrm{MMD}$ & 10,000 & 92.020 $\pm$ 3.535 & 53.774 $\pm$ 3.013 & 0.776 $\pm$ 0.014\\
    \bottomrule
    \end{tabular}
    \label{tab:mol_results}
   % \vskip -0.1in
\end{table*}
\fi 
\begin{figure}[ht!]
    \centering
    \vspace{-0.2cm}
    \includegraphics[width=0.45\columnwidth]{images/qed_step0.png}
    \includegraphics[width=0.45\columnwidth]{images/qed_step100.png}
    \caption{\textbf{Histograms of QED} values for the decoded SMILES strings corresponding to  $t=0$ and $t=T=100$ for the JKO-ICNN experiment ( $\textup{D}=\mathrm{Sinkhorn}$, $\lambda_2$=10,000).
    The shift to the right in the QED distribution corresponds to increased drug-likeness of the decoded molecule.}
    \label{fig:qed_hist}
%\vskip -0.21in
\end{figure}

\begin{table}[ht!]
    \centering
    \caption{\textbf{Computational amortization gains.}
    Comparison between re-use of maps calculated from JKO-ICNN flow and the direct optimization baseline applied to various sizes of embedding point clouds.
    For each setup, we report median QED for the final point cloud of embeddings from the respective flows and the Sinkhorn divergence between the initial and final point clouds (Final SD).
    We observe a linear trend in speed-up when re-using JKO-ICNN maps.
    % In the last two columns, we report the time taken for the direct optimization flow and the re-use of the maps from JKO-ICNN to a new set of points.
    % Speedup for each point cloud size is calculated as time taken for direct optimization baseline divided by time taken for re-use of JKO-ICNN maps.
    }
    \begin{tabular}{l | c c | c c}
    \toprule
    Size & QED Median & Final SD & Time (s) & Speedup \\
    \midrule
    \multicolumn{5}{l}{\textit{Baseline}}\\
    1,000 & 0.789 & 17.134 & 1.416 & \textemdash\\
    2,000 & 0.795 & 17.333 & 1.550 & \textemdash\\
    3,000 & 0.791 & 17.255 & 2.300 & \textemdash\\
    4,000 & 0.790 & 17.238 & 3.433 & \textemdash\\
    5,000 & 0.792 & 17.212 & 4.696 & \textemdash\\
    \multicolumn{5}{l}{\textit{JKO-ICNN maps}}\\
    1,000 & 0.778 & 1.739 & 0.086 & 1.330\\
    2,000 & 0.773 & 1.440 & 0.086 & 1.464\\
    3,000 & 0.771 & 1.363 & 0.086 & 2.213\\
    4,000 & 0.767 & 1.373 & 0.086 & 3.347\\
    5,000 & 0.764 & 1.384 & 0.088 & 4.608\\
    \bottomrule
    \end{tabular}
    \label{tab:amortization}
\end{table}

\paragraph{Evaluation}
We fixed $\lambda_1 = 1$ for all experiments, and used either $\mathrm{Sinkhorn}$ or $\mathrm{MMD}$ for $\textup{D}$. The weight $\lambda_2$ on $\textup{D}$ was set to either 1,000 or 10,000.
We start JKO with an initial cloud point $\rho_0$ of embedding that have QED < 0.7 randomly sampled from the MOSES test set.
In the Table \ref{tab:mol_results}, we report several measurements.
First is validity, which is the proportion of the decoded embeddings that have valid SMILES strings according to RDKit.
Of the valid strings, we calculate the percent that are unique.
Finally, we use RDKit to get the QED annotation of the decoded embeddings and report median values for the point cloud.
We re-ran experiments five times with different random seed initializations and report means and standard deviations. %in order to report means and plus/minus standard deviations for each measurement.
In the first row of Table \ref{tab:mol_results}, we report the initial values for the point cloud at time $t=0$.
In the last four rows of the table, we report the measurements for different hyperparameter configurations at the end of the JKO scheme for  $t=T=100$.
We see that the JKO-ICNN is able to optimize the functional objective and leads to molecules that satisfy low energy potential, i.e.~with improved drug-likeness.
The results are stable across different runs as can be seen from the reported standard deviations from the different random initializations.
We notice that $\mathrm{Sinkhorn}$ divergence with $\lambda_2=$10,000 prevents mode collapse and preserves uniqueness of the transported embedding via JKO-ICNN.
While $\mathrm{MMD}$ yields higher drug-likeness, it leads to a deterioration in uniqueness.
Using $\mathrm{Sinkhorn}$ allows for a matching between the transformed point cloud and the original one, which preserves better uniqueness than $\mathrm{MMD}$, which merely matches mean embeddings of the distributions.
Finally, in Figure \ref{fig:qed_hist} we display the histograms of the QED values for the decoded SMILES strings corresponding to the point clouds at time step $t=0$ and $t=T=100$ for $\textup{D}=\mathrm{Sinkhorn}$, $\lambda_2$=10,000. 

\paragraph{Comparison with direct optimization}
We also compare the JKO-ICNN flow to a baseline approach that optimizes the same functional objective via direct gradient descent on the molecule embeddings.
Formally, this baseline approach is described by the process:
$dX^i_t = -\nabla V(X^i_t)dt - \lambda_2 \nabla \textup{D}(\frac{1}{N}\sum_{i=1}^{N}\delta_{X^i_t},\rho_0), i=1 \dots N$, which we discretize using either vanilla gradient descent or \textsc{adam} updates.
In order to ensure a `fair shot’ at competing with our JKO-ICNN approach, we run a grid search over various hyperparameters, including optimizer (\textsc{sgd} or \textsc{adam}), learning rate, and $\lambda_2.$
While the full grid search results are available in Table \ref{tab:baseline_grid_search} in Appendix \ref{app:mol-pde}, we reproduce a selection of hyperparameter configurations in Table \ref{tab:baseline_comparison} to illustrate several key points.
\begin{table*}[ht!]
\vskip -0.1in
    \centering
    \caption{\textbf{Direct optimization baseline.}
    Comparison between JKO-ICNN (first row) and the direct optimization baseline.
    For each setup, we report validity, uniqueness, and median QED for the final point cloud of embeddings from the respective flows.
    We also report the Sinkhorn divergence between the initial and final point clouds (Final SD).
    Each measurement value cell contains mean values $\pm$ one standard deviation for five repeated runs with different random initialization seeds.
    The initial cloud point is presented in the first row.
    The best JKO-ICNN flow is reproduced in the second row.}
    %\small
    \begin{tabular}{l l | c c c c}
    \toprule
    $\lambda_2$ & LR & Validity & Uniqueness & QED Median & Final SD\\
    \midrule
    $\rho_0$\\
    N/A & N/A & 100.000 $\pm$ 0.000 & 99.980 $\pm$ 0.045 & 0.630 $\pm$ 0.001 & N/A\\
    \midrule\midrule
    \multicolumn{2}{l}{\textit{JKO-ICNN}}\\
    $1\mathrm{e}^{4}$ & $1\mathrm{e}^{-4}$ & 93.940 $\pm$ 0.336 & 100.000 $\pm$ 0.000 & 0.750 $\pm$ 0.001 & 0.620 $\pm$ 0.010\\
    \midrule\midrule
    \multicolumn{2}{l}{\textit{Baseline} - \textsc{sgd}}\\
    0 & $5\mathrm{e}^{-1}$ & 43.440 $\pm$ 1.092 & 100.000 $\pm$ 0.000 & 0.772 $\pm$ 0.004 & 9792.93 $\pm$ 76.913\\
    1 & $5\mathrm{e}^{-1}$ & 49.440 $\pm$ 1.128 & 100.000 $\pm$ 0.000 & 0.768 $\pm$ 0.006 & 8881.38 $\pm$ 69.736 \\
    $1\mathrm{e}^{3}$ & $5\mathrm{e}^{-1}$ & 87.240 $\pm$ 0.777 & 100.000 $\pm$ 0.000 & 0.767 $\pm$ 0.002 & 2515.08 $\pm$ 49.870 \\
    \multicolumn{2}{l}{\textit{Baseline} - \textsc{adam}}\\
    0 & $1\mathrm{e}^{-1}$ & 92.080 $\pm$ 0.973 & 100.000 $\pm$ 0.000 & 0.793 $\pm$ 0.005 & 18.261 $\pm$ 0.134\\
    0 & $1\mathrm{e}^{-2}$ & 93.900 $\pm$ 0.781 & 99.979 $\pm$ 0.048 & 0.758 $\pm$ 0.006 & 1.650 $\pm$ 0.006\\
    1 & $1\mathrm{e}^{-1}$ & 91.200 $\pm$ 0.539 & 99.978 $\pm$ 0.049 & 0.792 $\pm$ 0.005 & 17.170 $\pm$ 0.097\\
    $1\mathrm{e}^{3}$ & $1\mathrm{e}^{-1}$ & 99.980 $\pm$ 0.045 & 99.980 $\pm$ 0.045 & 0.630 $\pm$ 0.001 & 0.077 $\pm$ 0.003\\
    $1\mathrm{e}^{4}$ & $1\mathrm{e}^{-1}$ & 99.900 $\pm$ 0.122 & 99.980 $\pm$ 0.045 & 0.630 $\pm$ 0.001 & 0.240 $\pm$ 0.019\\
    \bottomrule
    \end{tabular}
    \label{tab:baseline_comparison}
\end{table*}

First, we note that the direct optimization baseline performs poorly when the $\lambda_2$ weight is at, or near that used in the JKO-ICNN experiment (10,000).
The only baseline configurations that are able to  meaningfully increase the median QED are those where $\lambda_2$ is orders of magnitude smaller than 10,000, i.e., those where the objective is essentially only QED.
This means that the direct optimization approach fails at accomplishing the joint goals of the objective function: increasing the QED attribute of the decoded molecules while staying close to the original set of embeddings.
For comparison, we show the Sinkhorn divergence between the final embedding set and the original molecule embeddings (reproduced in the first row of Table \ref{tab:baseline_comparison}) in the last column of the table (Final SD).
For JKO-ICNN (reproduced in the second row of Table \ref{tab:baseline_comparison} for reference), this final Sinkhorn divergence is up to several orders of magnitude smaller compared to direct optimizations that are able to successfully increase median QED.
From an application point of view, this is significant because, for example, in the drug re-purposing setting it is often crucial to stay close to the original set of points.
We also find that overall the direct optimization method on particles is quite sensitive to the choice of hyperparameters, something that we did not observe with JKO-ICNN.
We believe that this direct optimization comparison bolsters the claim that our JKO-ICNN approach is useful in real world, high-dimensional settings.

\paragraph{Benefit of computational amortization}
To further demonstrate the usefulness of our approach, we show that the maps calculated at each step of the JKO-ICNN flow can be re-used to transport a new set of embeddings with similar gains in QED distribution, without having to retrain the flow.
In Table \ref{tab:amortization}, we compare the results and computation time for the the best direct optimization hyperparameter configuration found during the grid search (Optimizer: \textsc{adam}, LR: 0.1, $\lambda_2$: 1) vs. re-using the maps found during the JKO-ICNN flow applied to a new set of embeddings.
We perform this comparison for various sample sizes of initial point clouds.
The linear scaling of the speedup of using the JKO-ICNN map relative to direct optimization underscores a major benefit of our approach, namely that one can solve the JKO-ICNN flow on one set of embeddings, save the map weights to disk, and effectively amortize the computational cost across any new set of embeddings that one wishes to transport.
This is a key advantage of our approach relative to the direct optimization baseline, which needs to be re-optimized for each new set of embeddings.
